Detecting Ransomware Execution in a Timely Manner

Ransomware has been an ongoing issue since the early 1990s. In recent times ransomware has spread from traditional computational resources to cyber-physical systems and industrial controls. We devised a series of experiments in which virtual instances are infected with ransomware. We instrumented the instances and collected resource utilization data across a variety of metrics (CPU, Memory, Disk Utility). We design a change point detection and learning method for identifying ransomware execution. Finally we evaluate and demonstrate its ability to detect ransomware efficiently in a timely manner when trained on a minimal set of samples. Our results represent a step forward for defense, and we conclude with further remarks for the path forward.

==> Sections/Results.tex <==
\section*{Experimental Collected Results}
We previously defined the experimental setup and in table~\ref{tbl:experimentsetdecomp} we decompose the experiments and its system usage.    The following time series plots illustrate the system under test:

\subsection*{\textbf{Normal Usage}} 
In figure~\ref{fig:normaltimeseries} Normal System Usage.  The system is executing typical user software such as a web browser or an editor.   

\begin{figure}
	\centering
	\begin{subfigure}{
			\includegraphics[width=0.47\linewidth]{PNGFigs/pngupdates/normaldisk.png}}
	\end{subfigure} 
		\begin{subfigure}{
			\includegraphics[width=0.47\linewidth]{PNGFigs/pngupdates/normalmemory.png}}
	\end{subfigure}    
	\hfill
	\caption{Normal memory and disk utilization as a user is using the system via performing activities such as web browsing and documentation.}
	\label{fig:normaltimeseries}
\end{figure}



As expected CPU, Memory and Disk utilization follows a pattern of activity consistent of normal system usage.  We do not notice a spike in activity and notice a series of downtime. As previously mentioned, in this experiment ransomware was not present on the system.

\subsection*{\textbf{Application Only}}
In figure~\ref{fig:apponly} is the time series graphs for parallel random execution of applications corresponding to the null hypothesis $H_0$. In the graph only one instance once chosen RANSOM3 where application usage occurred almost immediately after boot since $t_i$ was set randomly for a minimal time.

%\begin{figure}[h]
%	\begin{center}
%		\includegraphics[width=1\linewidth]{PNGFigs/apponly.png}
%	\end{center}
%	\caption{Parallel Application Only Execution}
%	\label{fig:apponly}
%\end{figure}

\begin{figure}
	\centering
	\begin{subfigure}{
			\includegraphics[width=0.47\linewidth]{PNGFigs/pngupdates/appdisk.png}}
	\end{subfigure} 
	\begin{subfigure}{
			\includegraphics[width=0.47\linewidth]{PNGFigs/pngupdates/apponlymemory.png}}
	\end{subfigure}    
	\hfill
	\caption{temporary caption}
	\label{fig:apponly}
\end{figure}



The results in figure~\ref{fig:apponly} correspond to the proposed experiment in figure~\ref{fig:nonransome}.  Memory, CPU, and Disk Usage seemed consistent post execution.  We note randomizing execution start time did not effect the overall impact to the aforementioned resource utilization.  


\subsection*{\textbf{Application and Sequential Ransomware Usage}}
Add in explanation...0

%\begin{figure}[h]
%	\begin{center}
%		\includegraphics[width=1\linewidth]{PNGFigs/seqwransome.png}
%	\end{center}
%	\caption{Random Time Initial Simultaneous Application Usage}
%	\label{fig:sequential}
%\end{figure}


\begin{figure}[h]
	\centering
	\begin{subfigure}{
			\includegraphics[width=\linewidth]{PNGFigs/pngupdates/sequentialdisk.png}}
	\end{subfigure}
	 
	\begin{subfigure}{
			\includegraphics[width=\linewidth]{PNGFigs/pngupdates/sequentialmemory.png}}
	\end{subfigure}    
	\hfill
	\caption{temporary caption}
	\label{fig:sequential}
\end{figure}

\subsection*{\textbf{Application and Parallel Ransomware Usage}}
Add in explanation...

\begin{figure}
	\centering
	\begin{subfigure}{
			\includegraphics[width=\linewidth]{PNGFigs/pngupdates/paralleldisk.png}}
	\end{subfigure} 
	\\
	\begin{subfigure}{
			\includegraphics[width=\linewidth]{PNGFigs/pngupdates/parallelmemory.png}}
	\end{subfigure}    
	\hfill
	\caption{temporary caption}
	\label{fig:parallel}
\end{figure}


\subsection*{\textbf{Ransomware Usage}}
A series of tests were conducted where ransomware was added to a series of guest operating systems as summarized by the experimental setup in table~\ref{tbl:experimentsetdecomp}.  At the point of execution of ransomware memory, cpu and disk activity are highly effected until the completion of encrypting files.


%\begin{figure}[h]
%	\begin{center}
%		\includegraphics[width=1\linewidth]{PNGFigs/ransomwareusage.png}
%	\end{center}
%	\caption{Ransomware Time Series Usage}
%	\label{fig:ransomwaretimeseries}
%\end{figure}

\begin{figure}
	\centering
	\begin{subfigure}{
			\includegraphics[width=\linewidth]{PNGFigs/pngupdates/ransomdisk.png}}
	\end{subfigure}
	 
	\begin{subfigure}{
			\includegraphics[width=\linewidth]{PNGFigs/pngupdates/ransommemory.png}}
	\end{subfigure}    
	\hfill
	\caption{temporary caption}
	\label{fig:ransomwaretimeseries}
\end{figure}


In the ransomware time series graphs illustrated in figure~\ref{fig:ransomwaretimeseries} CPU, Memory and Disk utilization is noticeably impacted when encryption is occurring.  This led us to conclude that a cross validation technique is needed when building the detector.    

%\subsection*{\textbf{Machine Learning Results}}
%\todo[inline]{Possibly include a figure of the decision tree and PCA analysis, Let me run these when new data is avalible as they will look better}

\subsection*{\textbf{Hypothesis Testing Results}}
Defined in the section \textit{Research Question and Hypothesis} and restated in the hypothesis in table~\ref{tbl:hypothesistesting}.

\begin{researchquestion}
	Can Machine Learning Provide Sufficient Detection Performance to Allow for Preventative Actions Prior to Data or Services Being Held Hostage?
\end{researchquestion}


%\todo[inline, color=green] {\textbf{ Needed for this section:}\\
%		Detection time and performance: we need to compare the detection time to the execution period of ransomware\\
%		Linkages to hypothesis / null hypothesis statements in table~\ref{tbl:hypothesistesting}\\
%		Conclusion of if the analysis was not conducted in a an enviornment such as Julia / Python (Scikit learn) and straight C that the performance gains could make the approach more viable in detection and prevention
%	}



\begin{table*}[!ht]
	\caption{Hypothesis Testing Results}
	\label{tbl:hypothesistesting}
	\centering
	\begin{tabular}{cll}
		\rowcolor[HTML]{C0C0C0} 
		\textbf{Hypothesis}                & \multicolumn{1}{c}{\cellcolor[HTML]{C0C0C0}\textbf{Hypothesis Statement}}                                                                                                                  & \multicolumn{1}{c}{\cellcolor[HTML]{C0C0C0}\textbf{Proven | Disproven}}                                                                     \\
		H1-Accuracy                        & \begin{tabular}[c]{@{}l@{}}A machine learning algorithm will be able to detect the \\ execution of ransomware with sufficient accuracy to\\  allow for preventative actions.\end{tabular}  & \textbf{\begin{tabular}[c]{@{}l@{}}(THIS IS WHERE WE WOULD \\ STATE WHICH SECTION IT IS \\ PROVEN / DISPROVEN IN OUR\\ PAPER)\end{tabular}} \\
		\rowcolor[HTML]{EFEFEF} 
		H2-Performance                     & \begin{tabular}[c]{@{}l@{}}A machine learning algorithm will be able to detect the\\ execution of ransomware in a sufficient time period to\\ allow for preventative actions.\end{tabular} &                                                                                                                                             \\
		H3-Features                        & \begin{tabular}[c]{@{}l@{}}There are significant features that can be used to\\  determine if ransomware is being actively executed.\end{tabular}                                          &                                                                                                                                             \\
		\rowcolor[HTML]{C0C0C0} 
		\textbf{Null Hypothesis}           & \multicolumn{1}{c}{\cellcolor[HTML]{C0C0C0}\textbf{Null Hypothesis Statement}}                                                                                                             & \multicolumn{1}{c}{\cellcolor[HTML]{C0C0C0}}                                                                                                \\
		H$_0$1-Accuracy                     & \begin{tabular}[c]{@{}l@{}}A machine learning algorithm will not have\\  sufficient accuracy to detect ransomware execution.\end{tabular}                                                  &                                                                                                                                             \\
		\rowcolor[HTML]{EFEFEF} 
		H$_0$2-Performance                  & \begin{tabular}[c]{@{}l@{}}A machine learning algorithm will not detect\\  ransomware execution in a sufficent time period\\  to allow for preventative actions.\end{tabular}              &                                                                                                                                             \\
		\multicolumn{1}{l}{H$_0$3-Accuracy} & \begin{tabular}[c]{@{}l@{}}There is not significant features that can be\\  used to determine if ransomware is being actively\\  executed.\end{tabular}                                    &                                                                                                                                            
	\end{tabular}
\end{table*}
